Giving BERT a Calculator: Finding Operations and Arguments with Reading Comprehension

Reading comprehension models have been successfully applied to extractive text answers, but it is unclear how best to generalize these models to abstractive numerical answers. We enable a BERT-based reading comprehension model to perform lightweight numerical reasoning. We augment the model with a predefined set of executable 'programs' which encompass simple arithmetic as well as extraction. Rather than having to learn to manipulate numbers directly, the model can pick a program and execute it. On the recent Discrete Reasoning Over Passages (DROP) dataset, designed to challenge reading comprehension models, we show a 33% absolute improvement by adding shallow programs. The model can learn to predict new operations when appropriate in a math word problem setting (Roy and Roth, 2015) with very few training examples.

==> derivations_distribution_table.tex <==



\begin{table}[t]
\centering
\small
\begin{tabular}{@{}l ccccc@{}}
\toprule
     & 1 & 2  & 3 & 4 & 5+ \\
  Op & (65\%) & (7.8\%) & (4.8\%) & (3.0\%) & (1.2\%) \\
\midrule
Span & 49 & - & - & - & - \\
2 Spans & 5.8 & - & - & - & - \\
3+ Spans & 3.2 & - & - & - & - \\
ID & 5.7 & 25 & 24 & 17 & 9 \\
Sum2 & 4.1 & 16 & 11 & 21 & 21 \\
Sum3 & 2.6 & - & - & - & - \\
Diff2 & 13 & 50 & 63 & 59 & 69 \\
Diff100 & 17 & 7.9 & 1.3 & 2.1 & 1 \\
\bottomrule
\end{tabular}
\caption{
Distribution of number of derivations and operation type for the DROP training (or dev?) set.
}
\label{tab:deriv-distrib}
\end{table}


